ToMBench: Benchmarking Theory of Mind in Large Language Models

Theory of Mind (ToM) is the cognitive capability to perceive and ascribe mental states to oneself and others. Recent research has sparked a debate over whether large language models (LLMs) exhibit a form of ToM. However, existing ToM evaluations are hindered by challenges such as constrained scope, subjective judgment, and unintended contamination, yielding inadequate assessments. To address this gap, we introduce ToMBench with three key characteristics: a systematic evaluation framework encompassing 8 tasks and 31 abilities in social cognition, a multiple-choice question format to support automated and unbiased evaluation, and a build-from-scratch bilingual inventory to strictly avoid data leakage. Based on ToMBench, we conduct extensive experiments to evaluate the ToM performance of 10 popular LLMs across tasks and abilities. We find that even the most advanced LLMs like GPT-4 lag behind human performance by over 10% points, indicating that LLMs have not achieved a human-level theory of mind yet. Our aim with ToMBench is to enable an efficient and effective evaluation of LLMs' ToM capabilities, thereby facilitating the development of LLMs with inherent social intelligence.

==> tables/ability-results-emotion.tex <==
\begin{table*}[h]
\vspace{0mm}
\small
%\scriptsize
%\footnotesize
\renewcommand\arraystretch{1.1}
\setlength{\abovecaptionskip}{0mm}
\setlength{\belowcaptionskip}{5mm}
\centering
\setlength{\tabcolsep}{2mm}
% \scalebox{0.98}{
\resizebox{1.\textwidth}{!}{
\begin{tabular}{ccccccccccccccc}
	& \multicolumn{2}{c}{Typical emotional reactions} & \multicolumn{2}{c}{Atypical emotional reactions} & \multicolumn{2}{c}{Discrepant emotions} & \multicolumn{2}{c}{Mixed emotions} & \multicolumn{2}{c}{Hidden emotions} & \multicolumn{2}{c}{Moral emotions} & \multicolumn{2}{c}{Emotion regulation} \\
	ChatGLM3-6B              & 0.89                   & 0.71                   & 0.33                    & 0.23                   & 0.525              & 0.35               & 0.6              & 0.35            & 0.55             & 0.463            & 0.55             & 0.5             & 0.4                & 0.35              \\
	LLaMA2-Chat-13B          & 0.63                   & 0.83                   & 0.33                    & 0.3                    & 0.275              & 0.475              & 0.525            & 0.525           & 0.4              & 0.463            & 0.275            & 0.625           & 0.25               & 0.35              \\
	Baichuan2-Chat-13B       & 0.84                   & 0.86                   & 0.42                    & 0.36                   & 0.4                & 0.55               & 0.55             & 0.525           & 0.625            & 0.525            & 0.675            & 0.55            & 0.4                & 0.35              \\
	Mistral-7B               & 0.84                   & 0.83                   & 0.54                    & 0.49                   & 0.425              & 0.475              & 0.55             & 0.65            & 0.55             & 0.6              & 0.575            & 0.775           & 0.3                & 0.25              \\
	Mixtral-8x7B             & 0.89                   & 0.73                   & 0.52                    & 0.48                   & 0.575              & 0.65               & 0.475            & 0.35            & 0.675            & 0.6              & 0.775            & 0.8             & 0.4                & 0.35              \\
	Qwen-Chat-14B            & 0.96                   & 0.89                   & 0.59                    & 0.5                    & 0.625              & 0.65               & 0.6              & 0.625           & 0.75             & 0.688            & 0.7              & 0.75            & 0.45               & 0.5               \\
	GPT-3.5-0613             & 0.91                   & 0.9                    & 0.54                    & 0.52                   & 0.525              & 0.675              & 0.3              & 0.575           & 0.588            & 0.65             & 0.625            & 0.775           & 0.6                & 0.5               \\
	GPT-3.5-1106             & 0.91                   & 0.86                   & 0.64                    & 0.56                   & 0.625              & 0.7                & 0.375            & 0.45            & 0.588            & 0.625            & 0.725            & 0.7             & 0.45               & 0.35              \\
	GPT-4-0613               & 0.96                   & 0.9                    & 0.63                    & 0.49                   & 0.9                & 0.85               & 0.7              & 0.65            & 0.887            & 0.8              & 0.9              & 0.85            & 0.55               & 0.5               \\
	GPT-4-1106               & 0.97                   & 0.94                   & 0.64                    & 0.55                   & 0.9                & 0.925              & 0.6              & 0.65            & 0.825            & 0.787            & 0.825            & 0.9             & 0.55               & 0.55              \\
	ChatGLM3-6B + CoT        & 0.89                   & 0.79                   & 0.46                    & 0.29                   & 0.575              & 0.45               & 0.475            & 0.55            & 0.487            & 0.438            & 0.525            & 0.55            & 0.3                & 0.2               \\
	LLaMA2-Chat-13B + CoT    & 0.67                   & 0.81                   & 0.37                    & 0.32                   & 0.375              & 0.5                & 0.4              & 0.4             & 0.463            & 0.487            & 0.5              & 0.55            & 0.25               & 0.3               \\
	Baichuan2-Chat-13B + CoT & 0.83                   & 0.81                   & 0.38                    & 0.33                   & 0.375              & 0.525              & 0.575            & 0.45            & 0.55             & 0.438            & 0.6              & 0.625           & 0.3                & 0.3               \\
	Mistral-7B + CoT         & 0.84                   & 0.8                    & 0.5                     & 0.48                   & 0.5                & 0.575              & 0.5              & 0.65            & 0.475            & 0.6              & 0.625            & 0.7             & 0.2                & 0.25              \\
	Mixtral-8x7B + CoT       & 0.86                   & 0.67                   & 0.51                    & 0.51                   & 0.5                & 0.675              & 0.375            & 0.325           & 0.662            & 0.562            & 0.725            & 0.825           & 0.35               & 0.35              \\
	Qwen-Chat-14B + CoT      & 0.88                   & 0.85                   & 0.58                    & 0.48                   & 0.65               & 0.7                & 0.55             & 0.5             & 0.738            & 0.662            & 0.675            & 0.7             & 0.4                & 0.5               \\
	GPT-3.5-0613 + CoT       & 0.89                   & 0.73                   & 0.55                    & 0.56                   & 0.7                & 0.675              & 0.45             & 0.55            & 0.6              & 0.7              & 0.725            & 0.675           & 0.4                & 0.5               \\
	GPT-3.5-1106 + CoT       & 0.89                   & 0.83                   & 0.61                    & 0.54                   & 0.6                & 0.675              & 0.7              & 0.525           & 0.625            & 0.613            & 0.6              & 0.725           & 0.4                & 0.45              \\
	GPT-4-0613 + CoT         & 0.91                   & 0.89                   & 0.65                    & 0.53                   & 0.7                & 0.85               & 0.825            & 0.725           & 0.838            & 0.8              & 0.85             & 0.875           & 0.6                & 0.45              \\
	GPT-4-1106 + CoT         & 0.93                   & 0.9                    & 0.62                    & 0.55                   & 0.85               & 0.9                & 0.725            & 0.675           & 0.825            & 0.8              & 0.925            & 0.9             & 0.5                & 0.4              
\end{tabular}
}

\vspace{1mm}
\caption{Ability-oriented ToM performance of different LLMs models. 
}

\label{tab-cokelm}
\vspace{-6mm}
\end{table*}

==> tables/task-and-ability-results.tex <==
\begin{table*}[h]
	\vspace{0mm}
	\small
	%\scriptsize
	%\footnotesize
	\renewcommand\arraystretch{1.0}
	\setlength{\abovecaptionskip}{0mm}
	\setlength{\belowcaptionskip}{5mm}
	\centering
	\setlength{\tabcolsep}{0.82mm}
	% \scalebox{0.98}{
		\resizebox{1.\textwidth}{!}{
			\begin{tabular}{ccc|cccccccccc|cccccccccc}
				\toprule
				\multicolumn{23}{l}{\makecell[tl]{\textbf{Large Language Models}: (M0) ChatGLM3-6B ~~~ (M1) LLaMA2-13B-Chat ~~~ (M2) Baichuan2-13B-Chat ~~~ (M3) Mistral-7B ~~~ (M4) Mixtral-8x7B \\~~~ ~~~~ ~~~~ ~~~~ ~~~~ ~~~~ ~~~~ ~~~~ ~~~~~(M5) Qwen-14B-Chat ~ (M6) GPT-3.5-Turbo-0613 ~ (M7) GPT-3.5-Turbo-1106 ~~~ (M8) GPT-4-0613 ~ (M9) GPT-4-1106}} \\ \midrule
				\makecell{Task /\\Ability} &    Human      & Lang.   & M0     & M1     & M2     & M3     & M4     & M5     & M6     & M7     & M8      & M9      & \makecell{M0\\+\\CoT}     & \makecell{M1\\+\\CoT}     & \makecell{M2\\+\\CoT}     & \makecell{M3\\+\\CoT}     & \makecell{M4\\+\\CoT}     & \makecell{M5\\+\\CoT}     & \makecell{M6\\+\\CoT}     & \makecell{M7\\+\\CoT}     & \makecell{M8\\+\\CoT}      & \makecell{M9\\+\\CoT}    \\ \midrule
				\multicolumn{23}{l}{\makecell[tl]{\textbf{Task-Oriented Results}: \textbb{UOT}: Unexpected Outcome Test ~~\textbb{SIT}: Scalar Implicature Task ~~\textbb{PST}: Persuasion Story Task ~~\textbb{FBT}: False Belief Task \\ ~~~~~~ ~~~~~~ ~~~~~~ ~~~~~~ ~~~~~~ ~~~~~~\textbb{AST}: Ambiguous Story Task ~~~~~~~~\textbb{HT}: Hinting Test~~~~~~ ~~~~~~ ~~ ~~~~~\textbb{SST}: Strange Story Task~~~~~~~ \textbb{FRT}: Faux-pas Recognition Test}}  \\ \midrule
				
				\multirow{2}{*}{\textbb{UOT}}  &  & zh& 55.3	& 43.7	& 56.3	& 61.0	& 68.0	& 72.0	& 69.3	& 72.3	& 71.3	& \bestd{76.7}	& 58.7	& 45.3	& 54.3	& 61.0	& 65.3	& 65.3	& 62.3	& 68.7	& 72.3	& \bestc{76.3} \\
				&  & en & 44.3	& 52.7	& 53.7	& 58.0	& 58.7	& 63.7	& 63.3	& 66.0	& \bestd{71.3}	& 71.0	& 50.3	& 52.7	& 48.7	& 55.3	& 52.3	& 58.0	& 58.3	& 64.7	& 64.7	& \bestc{72.7} \\ \midrule
				\multirow{2}{*}{\textbb{SIT}} &  & zh& 24.5	& 28.0	& 27.5	& 28.0	& \bestd{49.5}	& 42.5	& 33.0	& 34.0	& 49.0	& 48.0	& 27.0	& 25.5	& 26.5	& 27.0	& 45.0	& 31.5	& 30.0	& 27.5	& 43.5	& \bestc{48.0} \\
				&  & en & 28.0	& 23.5	& 32.0	& 34.5	& 42.5	& 30.5	& 35.0	& 33.0	& 44.0	& \bestd{49.0}	& 26.5	& 23.5	& 23.0	& 28.0	& 29.5	& 31.0	& 26.5	& 35.0	& 54.0	& \bestc{55.0} \\ \midrule
				\multirow{2}{*}{\textbb{PST}} &  & zh& 44.0	& 38.0	& 48.0	& 49.0	& 45.0	& 50.0	& 52.0	& 57.0	& 58.0	& \bestd{61.0}	& 44.0	& 34.0	& 33.0	& 46.0	& 41.0	& 45.0	& 43.0	& 45.0	& 55.0	& \bestc{59.0} \\
				&  & en & 41.0	& 43.0	& 36.0	& 51.0	& 55.0	& 51.0	& 49.0	& 56.0	& 53.0	& \bestd{65.0}	& 41.0	& 39.0	& 34.0	& 42.0	& 39.0	& 44.0	& 48.0	& 54.0	& 52.0	& \bestc{55.0} \\ \midrule
				\multirow{2}{*}{\textbb{FBT}} &  & zh& 59.2	& 42.2	& 50.2	& 43.5	& 49.8	& 57.2	& 61.2	& 53.0	& 86.3	& \bestd{90.8}	& 56.5	& 41.3	& 44.8	& 47.2	& 53.7	& 51.3	& 57.8	& 57.5	& \bestc{90.3}	& 88.7 \\
				&  & en & 48.5	& 42.8	& 51.5	& 46.7	& 37.8	& 58.7	& 62.3	& 55.0	& 80.0	& \bestd{88.2}	& 51.2	& 43.0	& 44.2	& 47.0	& 43.8	& 54.7	& 64.0	& 56.3	& 80.8	& \bestc{86.8} \\ \midrule
				\multirow{2}{*}{\textbb{AST}} &  & zh& 48.0	& 38.0	& 56.0	& 52.5	& 71.0	& 65.5	& 63.5	& 59.0	& \bestd{84.0}	& 83.0	& 48.0	& 41.0	& 51.5	& 47.0	& 66.0	& 62.5	& 58.5	& 61.5	& \bestc{84.5}	& 84.0 \\
				&  & en & 41.0	& 47.5	& 50.5	& 51.0	& 69.5	& 64.0	& 63.5	& 60.5	& \bestd{78.0}	& 77.5	& 44.0	& 48.5	& 44.0	& 46.5	& 59.5	& 63.0	& 58.0	& 63.0	& 77.5	& \bestc{81.0} \\ \midrule
				\multirow{2}{*}{\textbb{HT}} &  & zh& 32.0	& 32.0	& 54.4	& 29.1	& 43.7	& 54.4	& 60.2	& 61.2	& 79.6	& \bestd{88.3}	& 37.9	& 28.2	& 53.4	& 30.1	& 44.7	& 47.6	& 41.7	& 46.6	& 78.6	& \bestc{89.3} \\
				&  & en & 36.9	& 48.5	& 58.3	& 43.7	& 55.3	& 56.3	& 53.4	& 64.1	& 76.7	& \bestd{82.5}	& 42.7	& 43.7	& 49.5	& 37.9	& 54.4	& 48.5	& 41.7	& 51.5	& 76.7	& \bestc{82.5} \\ \midrule
				\multirow{2}{*}{\textbb{SST}} &  & zh& 58.0	& 58.2	& 50.1	& 53.1	& 51.4	& 60.0	& 72.0	& 72.5	& \bestd{83.0}	& 76.2	& 56.3	& 53.6	& 52.8	& 56.5	& 43.7	& 60.2	& 71.3	& 71.3	& \bestc{83.5}	& 76.9 \\
				&  & en & 37.8	& 58.0	& 50.4	& 60.0	& 53.8	& 59.5	& 66.1	& 69.0	& 81.1	& \bestd{84.0}	& 44.2	& 59.5	& 51.1	& 63.4	& 39.8	& 53.6	& 66.8	& 68.6	& 81.1	& \bestc{84.3} \\ \midrule
				\multirow{2}{*}{\textbb{FRT}} &  & zh& 55.2	& 47.9	& 61.6	& 63.6	& 62.5	& 72.7	& 66.8	& 68.8	& 76.6	& \bestd{78.6}	& 65.4	& 49.6	& 65.4	& 64.3	& 47.5	& 70.7	& 70.5	& 72.7	& 74.3	& \bestc{79.6} \\
				&  & en & 44.6	& 58.4	& 61.3	& 66.8	& 54.1	& 69.5	& 67.0	& 72.5	& 71.8	& \bestd{75.0}	& 51.4	& 62.1	& 52.5	& 64.1	& 54.3	& 67.7	& 70.4	& 70.9	& 73.6	& \bestc{75.2} \\ \midrule
			\multirow{2}{*}{\textbf{AVG.}} &  & zh& \cellcolor[gray]{0.9} 47.0	& \cellcolor[gray]{0.9} 41.0	& \cellcolor[gray]{0.9} 50.5	& \cellcolor[gray]{0.9} 47.5	& \cellcolor[gray]{0.9} 55.1	& \cellcolor[gray]{0.9} 59.3	& \cellcolor[gray]{0.9} 59.8	& \cellcolor[gray]{0.9} 59.7	& \cellcolor[gray]{0.9} 73.5	& \cellcolor[gray]{0.9} \bestd{75.3}	& \cellcolor[gray]{0.9} 49.2	& \cellcolor[gray]{0.9} 39.8	& \cellcolor[gray]{0.9} 47.7	& \cellcolor[gray]{0.9} 47.4	& \cellcolor[gray]{0.9} 50.9	& \cellcolor[gray]{0.9} 54.3	& \cellcolor[gray]{0.9} 54.4	& \cellcolor[gray]{0.9} 56.4	& \cellcolor[gray]{0.9} 72.8	& \cellcolor[gray]{0.9} \bestc{75.2} \\
			&   & en & \cellcolor[gray]{0.9}40.3	& \cellcolor[gray]{0.9} 46.8	& \cellcolor[gray]{0.9} 49.2	& \cellcolor[gray]{0.9} 51.5	& \cellcolor[gray]{0.9} 53.3	& \cellcolor[gray]{0.9} 56.7	& \cellcolor[gray]{0.9} 57.5	& \cellcolor[gray]{0.9} 59.5	& \cellcolor[gray]{0.9} 69.5	& \cellcolor[gray]{0.9} \bestd{74.0}	& \cellcolor[gray]{0.9} 43.9	& \cellcolor[gray]{0.9} 46.5	& \cellcolor[gray]{0.9} 43.4	& \cellcolor[gray]{0.9} 48.0	& \cellcolor[gray]{0.9} 46.6	& \cellcolor[gray]{0.9} 52.6	& \cellcolor[gray]{0.9} 54.2	& \cellcolor[gray]{0.9} 58.0	& \cellcolor[gray]{0.9} 70.1	& \cellcolor[gray]{0.9} \bestc{74.1} \\ \midrule
				
				\multicolumn{23}{l}{\makecell[tl]{\textbf{Ability-Oriented Results}: Averaged on categories due to space limitation. Please refer to Table \ref{tab-all-ability-results} in Appendix \ref{appendix-detailed-results} for all 31 mentalistic abilities.}}                                                                                   \\ \midrule
				
				\multirow{2}{*}{Emotion}    &  & zh &54.9	&38.4	&55.9	&54.0	&61.6	&66.8	&58.4	&61.6	&\bestd{79.0}	&75.9	&53.0	&43.3	&51.6	&52.0	&56.9	&63.9	&61.6	&63.2	&\bestc{76.8}	&\bestc{76.8} \\
				&  & en &42.2	&51.0	&53.1	&58.1	&56.6	&65.8	&65.6	&60.6	&72.0	&\bestd{75.7}	&46.7	&48.1	&49.7	&57.9	&56.0	&62.7	&62.7	&62.3	&73.1	&{73.2} \\ \midrule
				\multirow{2}{*}{Desire}    &  & zh &52.0	&39.2	&49.6	&48.7	&54.1	&57.0	&54.2	&57.1	&\bestd{72.2}	&67.5	&49.1	&37.4	&47.2	&46.9	&47.5	&57.3	&53.1	&54.7	&69.9	&\bestc{71.2} \\
				&  & en &40.7	&49.4	&46.0	&49.8	&51.2	&52.9	&53.4	&60.7	&60.2	&\bestd{69.7}	&43.7	&44.9	&37.5	&45.1	&41.5	&50.2	&52.1	&54.7	&\bestc{67.1}	&63.3 \\ \midrule
				\multirow{2}{*}{Intention}    &  & zh &52.0	&41.7	&63.5	&45.3	&60.1	&66.4	&58.2	&56.5	&\bestd{77.8}	&\bestd{77.8}	&54.8	&43.4	&51.3	&50.5	&57.9	&63.2	&65.4	&59.9	&\bestc{80.1}	&78.9 \\
				&  & en &35.9	&49.6	&52.2	&52.2	&64.1	&58.9	&61.0	&62.6	&66.1	&\bestd{84.7}	&49.8	&51.7	&47.8	&51.1	&55.3	&57.8	&63.8	&63.1	&71.5	&\bestc{77.9} \\ \midrule
				\multirow{2}{*}{Knowledge}    &  & zh &16.8	&22.4	&21.3	&33.1	&31.1	&37.9	&37.8	&30.4	&56.0	&\bestd{57.6}	&32.0	&28.7	&33.7	&33.4	&30.2	&41.0	&49.6	&34.6	&60.5	&\bestc{63.1} \\
				&  & en &22.0	&21.1	&20.9	&42.0	&27.1	&33.1	&36.3	&37.4	&48.1	&\bestd{52.1}	&28.9	&30.7	&19.3	&44.5	&33.2	&40.1	&43.3	&49.6	&57.5	&\bestc{60.4} \\ \midrule
				\multirow{2}{*}{Belief}    &  & zh &55.0	&46.7	&48.5	&47.2	&56.9	&62.2	&64.3	&60.6	&82.1	&\bestd{84.1}	&51.7	&43.8	&47.3	&50.9	&54.6	&56.2	&58.2	&61.9	&83.7	&\bestc{84.0} \\
				&  & en &44.5	&49.0	&49.8	&48.7	&48.1	&60.6	&61.4	&59.4	&76.1	&\bestd{82.8}	&48.6	&47.9	&45.2	&50.1	&44.3	&53.6	&58.7	&59.9	&76.4	&\bestc{83.6} \\ \midrule
				\multirow{2}{*}{NL Comm.}    &  & zh &49.8	&54.0	&46.2	&46.5	&50.9	&53.2	&76.8	&76.0	&\bestd{81.3}	&72.8	&55.8	&52.9	&52.4	&50.7	&44.6	&53.5	&70.0	&71.3	&\bestc{80.9}	&70.9 \\
				&  & en &38.5	&54.3	&50.1	&57.2	&57.9	&57.5	&66.9	&71.5	&81.5	&\bestd{84.0}	&40.1	&62.7	&47.5	&62.4	&45.5	&53.2	&71.6	&70.8	&82.2	&\bestc{83.0} \\ \midrule
				\multirow{2}{*}{\textbf{AVG.}}    &  & zh &\cellcolor[gray]{0.9}46.8	& \cellcolor[gray]{0.9}40.4	& \cellcolor[gray]{0.9}47.5	& \cellcolor[gray]{0.9}45.8	& \cellcolor[gray]{0.9}52.5	& \cellcolor[gray]{0.9}57.3	& \cellcolor[gray]{0.9}58.3	& \cellcolor[gray]{0.9}57.0	& \cellcolor[gray]{0.9}\bestd{74.7}	& \cellcolor[gray]{0.9}72.6	& \cellcolor[gray]{0.9}49.4	& \cellcolor[gray]{0.9}41.6	& \cellcolor[gray]{0.9}47.3	& \cellcolor[gray]{0.9}47.4	& \cellcolor[gray]{0.9}48.6	& \cellcolor[gray]{0.9}55.9	& \cellcolor[gray]{0.9}59.7	& \cellcolor[gray]{0.9}57.6	& \cellcolor[gray]{0.9}\bestc{75.3}	& \cellcolor[gray]{0.9}74.2 \\
				&   & en &\cellcolor[gray]{0.9}37.3	& \cellcolor[gray]{0.9}45.7	& \cellcolor[gray]{0.9}45.4	& \cellcolor[gray]{0.9}51.3	& \cellcolor[gray]{0.9}50.8	& \cellcolor[gray]{0.9}54.8	& \cellcolor[gray]{0.9}57.4	& \cellcolor[gray]{0.9}58.7	& \cellcolor[gray]{0.9}67.3	& \cellcolor[gray]{0.9}\bestd{74.8}	& \cellcolor[gray]{0.9}43.0	& \cellcolor[gray]{0.9}47.7	& \cellcolor[gray]{0.9}41.2	& \cellcolor[gray]{0.9}51.9	& \cellcolor[gray]{0.9}46.0	& \cellcolor[gray]{0.9}52.9	& \cellcolor[gray]{0.9}58.7	& \cellcolor[gray]{0.9}60.1	& \cellcolor[gray]{0.9}71.3	& \cellcolor[gray]{0.9}\bestc{73.6} \\ \bottomrule
				
			\end{tabular}
		}
		
		\vspace{1mm}
		\caption{Task- and ability-oriented ToM performance of LLMs. The best results of each under vanilla prompting are in \bestd{pink}, and those under CoT prompting are in \bestc{blue}.
		}
		
		\label{tab-results}
		\vspace{-6mm}
	\end{table*}

%\begin{table*}[h]
%	\vspace{0mm}
%	\small
%	%\scriptsize
%	%\footnotesize
%	\renewcommand\arraystretch{1.0}
%	\setlength{\abovecaptionskip}{0mm}
%	\setlength{\belowcaptionskip}{5mm}
%	\centering
%	\setlength{\tabcolsep}{0.5mm}
%	% \scalebox{0.98}{
%		\resizebox{1.\textwidth}{!}{
%			\begin{tabular}{ccc|cccccccccc|cccccccccc}
%				\toprule
%				\multicolumn{23}{l}{\makecell[tl]{(M0) ChatGLM3-6B ~~~ (M1) LLaMA2-13B-Chat ~~~ (M2) Baichuan2-13B-Chat ~~~ (M3) Mistral-7B ~~~ (M4) Mixtral-8x7B \\(M5) Qwen-14B-Chat ~ (M6) GPT-3.5-Turbo-0613 ~ (M7) GPT-3.5-Turbo-1106 ~~~ (M8) GPT-4-0613 ~ (M9) GPT-4-1106}} \\ \midrule
%				\makecell{Task /\\Ability} &    Human      & Lang.   & M0     & M1     & M2     & M3     & M4     & M5     & M6     & M7     & M8      & M9      & \makecell{M0\\+\\CoT}     & \makecell{M1\\+\\CoT}     & \makecell{M2\\+\\CoT}     & \makecell{M3\\+\\CoT}     & \makecell{M4\\+\\CoT}     & \makecell{M5\\+\\CoT}     & \makecell{M6\\+\\CoT}     & \makecell{M7\\+\\CoT}     & \makecell{M8\\+\\CoT}      & \makecell{M9\\+\\CoT}    \\ \midrule
%				\multicolumn{23}{l}{\makecell[tl]{\textbf{Task-Oriented Results}}}  \\ \midrule
%				
%				\multirow{2}{*}{\textbb{UOT}}  &  & zh& 55.3	& 43.7	& 56.3	& 61.0	& 68.0	& 72.0	& 69.3	& 72.3	& 71.3	& \bestd{76.7}	& 58.7	& 45.3	& 54.3	& 61.0	& 65.3	& 65.3	& 62.3	& 68.7	& 72.3	& \bestc{76.3} \\
%				&  & en & 44.3	& 52.7	& 53.7	& 58.0	& 58.7	& 63.7	& 63.3	& 66.0	& \bestd{71.3}	& 71.0	& 50.3	& 52.7	& 48.7	& 55.3	& 52.3	& 58.0	& 58.3	& 64.7	& 64.7	& \bestc{72.7} \\ \midrule
%				\multirow{2}{*}{\textbb{SIT}} &  & zh& 24.5	& 28.0	& 27.5	& 28.0	& \bestd{49.5}	& 42.5	& 33.0	& 34.0	& 49.0	& 48.0	& 27.0	& 25.5	& 26.5	& 27.0	& 45.0	& 31.5	& 30.0	& 27.5	& 43.5	& \bestc{48.0} \\
%				&  & en & 28.0	& 23.5	& 32.0	& 34.5	& 42.5	& 30.5	& 35.0	& 33.0	& 44.0	& \bestd{49.0}	& 26.5	& 23.5	& 23.0	& 28.0	& 29.5	& 31.0	& 26.5	& 35.0	& 54.0	& \bestc{55.0} \\ \midrule
%				\multirow{2}{*}{\textbb{PST}} &  & zh& 44.0	& 38.0	& 48.0	& 49.0	& 45.0	& 50.0	& 52.0	& 57.0	& 58.0	& \bestd{61.0}	& 44.0	& 34.0	& 33.0	& 46.0	& 41.0	& 45.0	& 43.0	& 45.0	& 55.0	& \bestc{59.0} \\
%				&  & en & 41.0	& 43.0	& 36.0	& 51.0	& 55.0	& 51.0	& 49.0	& 56.0	& 53.0	& \bestd{65.0}	& 41.0	& 39.0	& 34.0	& 42.0	& 39.0	& 44.0	& 48.0	& 54.0	& 52.0	& \bestc{55.0} \\ \midrule
%				\multirow{2}{*}{\textbb{FBT}} &  & zh& 59.2	& 42.2	& 50.2	& 43.5	& 49.8	& 57.2	& 61.2	& 53.0	& 86.3	& \bestd{90.8}	& 56.5	& 41.3	& 44.8	& 47.2	& 53.7	& 51.3	& 57.8	& 57.5	& \bestc{90.3}	& 88.7 \\
%				&  & en & 48.5	& 42.8	& 51.5	& 46.7	& 37.8	& 58.7	& 62.3	& 55.0	& 80.0	& \bestd{88.2}	& 51.2	& 43.0	& 44.2	& 47.0	& 43.8	& 54.7	& 64.0	& 56.3	& 80.8	& \bestc{86.8} \\ \midrule
%				\multirow{2}{*}{\textbb{AST}} &  & zh& 48.0	& 38.0	& 56.0	& 52.5	& 71.0	& 65.5	& 63.5	& 59.0	& \bestd{84.0}	& 83.0	& 48.0	& 41.0	& 51.5	& 47.0	& 66.0	& 62.5	& 58.5	& 61.5	& \bestc{84.5}	& 84.0 \\
%				&  & en & 41.0	& 47.5	& 50.5	& 51.0	& 69.5	& 64.0	& 63.5	& 60.5	& \bestd{78.0}	& 77.5	& 44.0	& 48.5	& 44.0	& 46.5	& 59.5	& 63.0	& 58.0	& 63.0	& 77.5	& \bestc{81.0} \\ \midrule
%				\multirow{2}{*}{\textbb{HT}} &  & zh& 32.0	& 32.0	& 54.4	& 29.1	& 43.7	& 54.4	& 60.2	& 61.2	& 79.6	& \bestd{88.3}	& 37.9	& 28.2	& 53.4	& 30.1	& 44.7	& 47.6	& 41.7	& 46.6	& 78.6	& \bestc{89.3} \\
%				&  & en & 36.9	& 48.5	& 58.3	& 43.7	& 55.3	& 56.3	& 53.4	& 64.1	& 76.7	& \bestd{82.5}	& 42.7	& 43.7	& 49.5	& 37.9	& 54.4	& 48.5	& 41.7	& 51.5	& 76.7	& \bestc{82.5} \\ \midrule
%				\multirow{2}{*}{\textbb{SST}} &  & zh& 58.0	& 58.2	& 50.1	& 53.1	& 51.4	& 60.0	& 72.0	& 72.5	& \bestd{83.0}	& 76.2	& 56.3	& 53.6	& 52.8	& 56.5	& 43.7	& 60.2	& 71.3	& 71.3	& \bestc{83.5}	& 76.9 \\
%				&  & en & 37.8	& 58.0	& 50.4	& 60.0	& 53.8	& 59.5	& 66.1	& 69.0	& 81.1	& \bestd{84.0}	& 44.2	& 59.5	& 51.1	& 63.4	& 39.8	& 53.6	& 66.8	& 68.6	& 81.1	& \bestc{84.3} \\ \midrule
%				\multirow{2}{*}{\textbb{FRT}} &  & zh& 55.2	& 47.9	& 61.6	& 63.6	& 62.5	& 72.7	& 66.8	& 68.8	& 76.6	& \bestd{78.6}	& 65.4	& 49.6	& 65.4	& 64.3	& 47.5	& 70.7	& 70.5	& 72.7	& 74.3	& \bestc{79.6} \\
%				&  & en & 44.6	& 58.4	& 61.3	& 66.8	& 54.1	& 69.5	& 67.0	& 72.5	& 71.8	& \bestd{75.0}	& 51.4	& 62.1	& 52.5	& 64.1	& 54.3	& 67.7	& 70.4	& 70.9	& 73.6	& \bestc{75.2} \\ \midrule
%				\multirow{2}{*}{\textbf{AVG.}} &  & zh& 47.0	& 41.0	& 50.5	& 47.5	& 55.1	& 59.3	& 59.8	& 59.7	& 73.5	& \bestd{75.3}	& 49.2	& 39.8	& 47.7	& 47.4	& 50.9	& 54.3	& 54.4	& 56.4	& 72.8	& \bestc{75.2} \\
%				&  & en & 40.3	& 46.8	& 49.2	& 51.5	& 53.3	& 56.7	& 57.5	& 59.5	& 69.5	& \bestd{74.0}	& 43.9	& 46.5	& 43.4	& 48.0	& 46.6	& 52.6	& 54.2	& 58.0	& 70.1	& \bestc{74.1} \\ \midrule
%				
%				\multicolumn{23}{l}{\makecell[tl]{\textbf{Ability-Oriented Results}}}                                                                                   \\ \midrule
%				
%				\multirow{2}{*}{Emotion}    &  & zh &54.9	&38.4	&55.9	&54.0	&61.6	&66.8	&58.4	&61.6	&\bestd{79.0}	&75.9	&53.0	&43.3	&51.6	&52.0	&56.9	&63.9	&61.6	&63.2	&\bestc{76.8}	&\bestc{76.8} \\
%				&  & en &42.2	&51.0	&53.1	&58.1	&56.6	&65.8	&65.6	&60.6	&72.0	&\bestd{75.7}	&46.7	&48.1	&49.7	&57.9	&56.0	&62.7	&62.7	&62.3	&73.1	&{73.2} \\ \midrule
%				\multirow{2}{*}{Desire}    &  & zh &52.0	&39.2	&49.6	&48.7	&54.1	&57.0	&54.2	&57.1	&\bestd{72.2}	&67.5	&49.1	&37.4	&47.2	&46.9	&47.5	&57.3	&53.1	&54.7	&69.9	&\bestc{71.2} \\
%				&  & en &40.7	&49.4	&46.0	&49.8	&51.2	&52.9	&53.4	&60.7	&60.2	&\bestd{69.7}	&43.7	&44.9	&37.5	&45.1	&41.5	&50.2	&52.1	&54.7	&\bestc{67.1}	&63.3 \\ \midrule
%				\multirow{2}{*}{Intention}    &  & zh &52.0	&41.7	&63.5	&45.3	&60.1	&66.4	&58.2	&56.5	&\bestd{77.8}	&\bestd{77.8}	&54.8	&43.4	&51.3	&50.5	&57.9	&63.2	&65.4	&59.9	&\bestc{80.1}	&78.9 \\
%				&  & en &35.9	&49.6	&52.2	&52.2	&64.1	&58.9	&61.0	&62.6	&66.1	&\bestd{84.7}	&49.8	&51.7	&47.8	&51.1	&55.3	&57.8	&63.8	&63.1	&71.5	&\bestc{77.9} \\ \midrule
%				\multirow{2}{*}{Knowledge}    &  & zh &16.8	&22.4	&21.3	&33.1	&31.1	&37.9	&37.8	&30.4	&56.0	&\bestd{57.6}	&32.0	&28.7	&33.7	&33.4	&30.2	&41.0	&49.6	&34.6	&60.5	&\bestc{63.1} \\
%				&  & en &22.0	&21.1	&20.9	&42.0	&27.1	&33.1	&36.3	&37.4	&48.1	&\bestd{52.1}	&28.9	&30.7	&19.3	&44.5	&33.2	&40.1	&43.3	&49.6	&57.5	&\bestc{60.4} \\ \midrule
%				\multirow{2}{*}{Belief}    &  & zh &55.0	&46.7	&48.5	&47.2	&56.9	&62.2	&64.3	&60.6	&82.1	&\bestd{84.1}	&51.7	&43.8	&47.3	&50.9	&54.6	&56.2	&58.2	&61.9	&83.7	&\bestc{84.0} \\
%				&  & en &44.5	&49.0	&49.8	&48.7	&48.1	&60.6	&61.4	&59.4	&76.1	&\bestd{82.8}	&48.6	&47.9	&45.2	&50.1	&44.3	&53.6	&58.7	&59.9	&76.4	&\bestc{83.6} \\ \midrule
%				\multirow{2}{*}{NL Comm.}    &  & zh &49.8	&54.0	&46.2	&46.5	&50.9	&53.2	&76.8	&76.0	&\bestd{81.3}	&72.8	&55.8	&52.9	&52.4	&50.7	&44.6	&53.5	&70.0	&71.3	&\bestc{80.9}	&70.9 \\
%				&  & en &38.5	&54.3	&50.1	&57.2	&57.9	&57.5	&66.9	&71.5	&81.5	&\bestd{84.0}	&40.1	&62.7	&47.5	&62.4	&45.5	&53.2	&71.6	&70.8	&82.2	&\bestc{83.0} \\ \midrule
%				\multirow{2}{*}{\textbf{AVG.}}    &  & zh &46.8	&40.4	&47.5	&45.8	&52.5	&57.3	&58.3	&57.0	&\bestd{74.7}	&72.6	&49.4	&41.6	&47.3	&47.4	&48.6	&55.9	&59.7	&57.6	&\bestc{75.3}	&74.2 \\
%				&  & en &37.3	&45.7	&45.4	&51.3	&50.8	&54.8	&57.4	&58.7	&67.3	&\bestd{74.8}	&43.0	&47.7	&41.2	&51.9	&46.0	&52.9	&58.7	&60.1	&71.3	&\bestc{73.6} \\ \bottomrule
%				
%			\end{tabular}
%		}
%		
%		\vspace{1mm}
%		\caption{Task- and ability-oriented ToM performance of LLMs. The best results under vanilla prompting are in \bestd{pink}, and those under CoT prompting are in \bestc{blue}. \textbf{Task-Oriented Results}: \textbb{UOT}: Unexpected Outcome Test ~~\textbb{SIT}: Scalar Implicature Task ~~\textbb{PST}: Persuasion Story Task ~~\textbb{FBT}: False Belief Task \\ ~~~~~~ ~~~~~~ ~~~~~~ ~~~~~~ ~~~~~~ ~~~~~~\textbb{AST}: Ambiguous Story Task ~~~~~~~~\textbb{HT}: Hinting Test~~~~~~ ~~~~~~ ~~ ~~~~~\textbb{SST}: Strange Story Task~~~~~~~ \textbb{FRT}: Faux-pas Recognition Test. Averaged on categories due to space limitation. Please refer to Table \ref{tab-all-ability-results} in Appendix \ref{appendix-detailed-results} for all 31 mentalistic abilities.
%		}
%		
%		\label{tab-results}
%		\vspace{-6mm}
%	\end{table*}
